Creating large Fock states and massively squeezed states in optics using systems with nonlinear bound states in the continuum

The quantization of the electromagnetic field leads directly to the existence of quantum mechanical states, called Fock states, with an exact integer number of photons. Despite these fundamental states being long-understood, and despite their many potential applications, generating them is largely an open problem. For example, at optical frequencies, it is challenging to deterministically generate Fock states of order two and beyond. Here, we predict the existence of a new effect in nonlinear optics, which enables the deterministic generation of large Fock states at arbitrary frequencies. The effect, which we call an n-photon bound state in the continuum, is one in which a photonic resonance (such as a cavity mode) becomes lossless when a precise number of photons n is inside the resonance. Based on analytical theory and numerical simulations, we show that these bound states enable a remarkable phenomenon in which a coherent state of light, when injected into a system supporting this bound state, can spontaneously evolve into a Fock state of a controllable photon number. This effect is also directly applicable for creating (highly) squeezed states of light, whose photon number fluctuations are (far) below the value expected from classical physics (i.e., shot noise). We suggest several examples of systems to experimentally realize the effects predicted here in nonlinear nanophotonic systems, showing examples of generating both optical Fock states with large n (n > 10), as well as more macroscopic photonic states with very large squeezing, with over 90% less noise (10 dB) than the classical value associated with shot noise.

==> n-photon BICs - PNAS/preamble.tex <==
%-----CHANGING CITATION APPEARANCE----
\setcitestyle{numbers,square,sort&compress} %We don't want the rmp citation style, but standard style square bracket, numbers style instead

%----KERNING-----
\usepackage{microtype} %For better kerning and symbol-stretching
\usepackage{xspace} %For the \xspace command

%----LOADING RELEVANT FONTS [TIMES ROMAN FOR PRB] -----
\usepackage{txfonts}  %Times Roman fonts
\usepackage{txfontsb} %Addition for txfonts, including old style numerals and greek
%					  %\usepackage{mathptmx} Also a Times Roman Font
%\usepackage{bm} %Bold math symbols with \bm{} (Greek and other symbols)
%\usepackage{mnsymbol} %For llangle and rrangle

%-----CROSS-REFERENCING-----
\usepackage{xr}

%-----COLOR AND GRAPHICS PACKAGES-----
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{calc,decorations.markings}

%-----SETTINGS FOR REFERENCES-----
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={blue!75!black!80!yellow},
    citecolor={blue!75!black!80!yellow},
    urlcolor={blue!75!black!80!yellow}
}

%-----PACKAGE FOR BOXED MULTI-LINE EQUATIONS-----
\usepackage{empheq}
\newcommand*\widefbox[1]{\fbox{\hspace{2em}#1\hspace{2em}}}

%-----CHANGE MARGINS OF DOCUMENT-----
\usepackage[top=1in, bottom=1.5in, left=1.4in, right=1.4in]{geometry} %Change margins

%-----SOME SETTINGS FOR MARGINPAR-----
%\usepackage{marginfix} %Should fix even more than mparhack, so use this instead unless you see something funky

\let\oldmarginpar\marginpar %This and the next line changes the fontsize
\def\marginpar#1{\oldmarginpar{\scriptsize #1}}
\setlength{\marginparwidth}{6.5em} %Changes the width of the note
\setlength{\marginparsep}{2em} %Probably enforces a minimum distance between marginpar-notes


%INCLUDING CLEVEREF PACKAGE FOR MORE CONVENIENT REFERENCING ABILITIES
\usepackage[capitalize,nameinlink]{cleveref}
\newcommand{\crefrangeconjunction}{\,--\,}
\crefname{subequations}{Eqs.}{Eqs.} %Specific changes to allow for Eqs.-wording when referring to a set of subequations. Label of subequations must include [subequations] as an option.
\Crefname{subequations}{Eqs.}{Eqs.}
\crefformat{subequations}{#2Eqs.~(#1)#3}
\Crefformat{subequations}{#2Eqs.~(#1)#3}
\crefname{page}{p.}{p.} %Changing from 'page' to 'p.'
\newcommand{\heqref}[1]{\hyperref[#1]{(\ref*{#1})}} %Alternative to \eqref, which works better with hyperlinks (whole thing is clickable)
\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable
\newcommand{\namedeqref}[2]{\hyperref[#2]{#1~(\ref*{#2})}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable


%-----PACKAGE TO ALLOW CHANGING OF ENUMERATE BULLETS-----
\usepackage{enumitem}

%-----COMMANDS-----
\newcommand{\vek}[1]{\mathbf{#1}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\qv}{\mathbf{q}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\nablav}{\boldsymbol{\nabla}}
\newcommand{\hxv}{\hat{\mathbf{x}}}
\newcommand{\hyv}{\hat{\mathbf{y}}}
\newcommand{\ef}{\epsilon_{\text{\textsc{f}}}}
\newcommand{\vf}{v_{\text{\textsc{f}}}}
\newcommand{\tsc}[1]{\text{\textsc{#1}}}
\newcommand{\kb}{k_\tsc{b}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ddb}[1]{\!\dd#1\,}
\newcommand{\dde}{\,\dd}
\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern.2pt}\sim\cr\noalign{\kern-2.5pt}}}}}

\newcommand{\spar}{_{\scriptscriptstyle\parallel}}
\newcommand{\kpar}{k_{\scriptscriptstyle\parallel}}
\newcommand{\kvpar}{\kv_{\scriptscriptstyle\parallel}}
\newcommand{\rpar}{r_{\scriptscriptstyle\parallel}}
\newcommand{\rvpar}{\rv_{\scriptscriptstyle\parallel}}
\newcommand{\vpar}{v_{\scriptscriptstyle\parallel}}
\newcommand{\vvpar}{\vv_{\scriptscriptstyle\parallel}}
\newcommand{\dperp}{d_{\perp}}
\newcommand{\dpar}{d_{\parallel}}
\newcommand{\iu}{\mathrm{i}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\sgn}{\operatorname{sgn}}

\newcommand{\pr}[1]{|#1\rangle\langle#1|}
\newcommand{\prsf}[1]{\mathsf{|#1\rangle\langle#1|}}

\newcommand{\Ev}{\mathbf{E}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Hv}{\mathbf{H}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\dv}{\mathbf{d}}
\newcommand{\hv}{\mathbf{h}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\Gv}{\mathbf{G}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\nv}{\hat{\mathbf{n}}}

%abbreviations
\newcommand{\ie}{i.e.\@\xspace} %Gobble-spaces of the "small" type (small is ensured by adding \@)
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}

==> preamble.tex <==
%-----CHANGING CITATION APPEARANCE----
\setcitestyle{numbers,square,sort&compress} %We don't want the rmp citation style, but standard style square bracket, numbers style instead

%----KERNING-----
\usepackage{microtype} %For better kerning and symbol-stretching
\usepackage{xspace} %For the \xspace command

%----LOADING RELEVANT FONTS [TIMES ROMAN FOR PRB] -----
\usepackage{txfonts}  %Times Roman fonts
\usepackage{txfontsb} %Addition for txfonts, including old style numerals and greek
%					  %\usepackage{mathptmx} Also a Times Roman Font
%\usepackage{bm} %Bold math symbols with \bm{} (Greek and other symbols)
%\usepackage{mnsymbol} %For llangle and rrangle

%-----CROSS-REFERENCING-----
\usepackage{xr}

%-----COLOR AND GRAPHICS PACKAGES-----
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{calc,decorations.markings}

%-----SETTINGS FOR REFERENCES-----
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={blue!75!black!80!yellow},
    citecolor={blue!75!black!80!yellow},
    urlcolor={blue!75!black!80!yellow}
}

%-----PACKAGE FOR BOXED MULTI-LINE EQUATIONS-----
\usepackage{empheq}
\newcommand*\widefbox[1]{\fbox{\hspace{2em}#1\hspace{2em}}}

%-----CHANGE MARGINS OF DOCUMENT-----
\usepackage[top=1in, bottom=1.5in, left=1.4in, right=1.4in]{geometry} %Change margins

%-----SOME SETTINGS FOR MARGINPAR-----
%\usepackage{marginfix} %Should fix even more than mparhack, so use this instead unless you see something funky

\let\oldmarginpar\marginpar %This and the next line changes the fontsize
\def\marginpar#1{\oldmarginpar{\scriptsize #1}}
\setlength{\marginparwidth}{6.5em} %Changes the width of the note
\setlength{\marginparsep}{2em} %Probably enforces a minimum distance between marginpar-notes


%INCLUDING CLEVEREF PACKAGE FOR MORE CONVENIENT REFERENCING ABILITIES
\usepackage[capitalize,nameinlink]{cleveref}
\newcommand{\crefrangeconjunction}{\,--\,}
\crefname{subequations}{Eqs.}{Eqs.} %Specific changes to allow for Eqs.-wording when referring to a set of subequations. Label of subequations must include [subequations] as an option.
\Crefname{subequations}{Eqs.}{Eqs.}
\crefformat{subequations}{#2Eqs.~(#1)#3}
\Crefformat{subequations}{#2Eqs.~(#1)#3}
\crefname{page}{p.}{p.} %Changing from 'page' to 'p.'
\newcommand{\heqref}[1]{\hyperref[#1]{(\ref*{#1})}} %Alternative to \eqref, which works better with hyperlinks (whole thing is clickable)
\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable
\newcommand{\namedeqref}[2]{\hyperref[#2]{#1~(\ref*{#2})}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable


%-----PACKAGE TO ALLOW CHANGING OF ENUMERATE BULLETS-----
\usepackage{enumitem}

%-----COMMANDS-----
\newcommand{\vek}[1]{\mathbf{#1}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\qv}{\mathbf{q}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\nablav}{\boldsymbol{\nabla}}
\newcommand{\hxv}{\hat{\mathbf{x}}}
\newcommand{\hyv}{\hat{\mathbf{y}}}
\newcommand{\ef}{\epsilon_{\text{\textsc{f}}}}
\newcommand{\vf}{v_{\text{\textsc{f}}}}
\newcommand{\tsc}[1]{\text{\textsc{#1}}}
\newcommand{\kb}{k_\tsc{b}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ddb}[1]{\!\dd#1\,}
\newcommand{\dde}{\,\dd}
\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern.2pt}\sim\cr\noalign{\kern-2.5pt}}}}}

\newcommand{\spar}{_{\scriptscriptstyle\parallel}}
\newcommand{\kpar}{k_{\scriptscriptstyle\parallel}}
\newcommand{\kvpar}{\kv_{\scriptscriptstyle\parallel}}
\newcommand{\rpar}{r_{\scriptscriptstyle\parallel}}
\newcommand{\rvpar}{\rv_{\scriptscriptstyle\parallel}}
\newcommand{\vpar}{v_{\scriptscriptstyle\parallel}}
\newcommand{\vvpar}{\vv_{\scriptscriptstyle\parallel}}
\newcommand{\dperp}{d_{\perp}}
\newcommand{\dpar}{d_{\parallel}}
\newcommand{\iu}{\mathrm{i}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\sgn}{\operatorname{sgn}}

\newcommand{\pr}[1]{|#1\rangle\langle#1|}
\newcommand{\prsf}[1]{\mathsf{|#1\rangle\langle#1|}}

\newcommand{\Ev}{\mathbf{E}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Hv}{\mathbf{H}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\dv}{\mathbf{d}}
\newcommand{\hv}{\mathbf{h}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\Gv}{\mathbf{G}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\nv}{\hat{\mathbf{n}}}

%abbreviations
\newcommand{\ie}{i.e.\@\xspace} %Gobble-spaces of the "small" type (small is ensured by adding \@)
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
